Polynomial Complex Ginzburg-Landau equations in almost periodic spaces

We consider Complex Ginzburg-Landau equations with a polynomial nonlinearity in the real line. We use splitting-methods to prove well-posedness for a subset of almost periodic spaces. Specifically, we prove that if the initial condition has multiples of an irrational phase, then the solution of the equation maintains those same phases.

==> def.tex <==

%\renewcommand{\thechapter}{\Roman{chapter}}


%%%%% EQUATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}

%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{corollary}{Corolario}[section]
%\newtheorem{lemma}{Lema}[section]
%\newtheorem{proposition}{Proposición}[section]
%\newtheorem{theorem}{Teorema}[section]

%%%%% demS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\renewenvironment{proof}[1][Demostraci\'on]{\noindent \textbf{#1.} }{\rule{0.5em}{0.5em}}

%%%%% DEFINITIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem{conjeture}{Conjetura}[section]
%\newtheorem{definition}{Definición}[section]
%\newtheorem{example}{Ejemplo}[section]
%\newtheorem{remark}{Observación}[section]
\newtheorem{exercise}{Ejercicio}[section]
{\swapnumbers\newtheorem{exercisestar}[exercise]{(*)}}
\newenvironment{sol}[1][\textbf{Solución:}]
{\noindent #1 \noindent \small}


%%%%% NUMERICAL SETS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}

%%%%% FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\abs}[1]{\ensuremath{\left\vert #1\right\vert}}
\newcommand{\ket}[1]{\ensuremath{\left| #1 \right\rangle}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand{\norm}[1]{\ensuremath{\left\|#1\right\|}}
\newcommand{\pa}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\pro}[2]{\ensuremath{\langle #1|#2 \rangle}}
\newcommand{\proo}[3]{\ensuremath{\langle #1|#2|#3 \rangle}}
\newcommand{\Rn}[1][n]{\ensuremath{\mathbb{R}^{#1}}}
\newcommand{\Cn}[1][n]{\ensuremath{\mathbb{C}^{#1}}}
\newcommand{\sgn}[1]{\ensuremath{\mathrm{sgn}\pa{#1}}}
\newcommand{\ran}[1]{\mathrm{Ran}\pa{#1}}
\newcommand{\tr}[1]{\mathop{\mathrm{tr}}\pa{#1}}

\newcommand{\hil}[1][X]{\ensuremath{\mathrm{#1}}}
\newcommand{\ham}[1][H]{\ensuremath{\mathcal{#1}}}
\newcommand{\kam}[1][H]{\ensuremath{\mathcal{#1}}}

\renewcommand{\Re}[1]{\ensuremath{\mathrm{Re}\left( #1\right)}}
\renewcommand{\Im}[1]{\mathrm{Im}\left( #1\right)}
\renewcommand{\exp}[1]{\mathrm{exp}\left( #1\right)}
%\renewcommand{\exp}[1]{e^{#1}}
\renewcommand{\cos}[1]{\mathrm{cos}\left( #1\right)}
\renewcommand{\sin}[1]{\mathrm{sen}\left( #1\right)}
%\newcommand{\id}{\mathds{1}}


\newcommand{\num}[3]{\ensuremath{#1\times 10^{#2}\,\mathrm{#3}}}
\newcommand{\al}{&\,}
